Habitat Synthetic Scenes Dataset (HSSD-200): An Analysis of 3D Scene Scale and Realism Tradeoffs for ObjectGoal Navigation

We contribute the Habitat Synthetic Scene Dataset, a dataset of 211 high-quality 3D scenes, and use it to test navigation agent generalization to realistic 3D environments. Our dataset represents real interiors and contains a diverse set of 18,656 models of real-world objects. We investigate the impact of synthetic 3D scene dataset scale and realism on the task of training embodied agents to find and navigate to objects (ObjectGoal navigation). By comparing to synthetic 3D scene datasets from prior work, we find that scale helps in generalization, but the benefits quickly saturate, making visual fidelity and correlation to real-world scenes more important. Our experiments show that agents trained on our smaller-scale dataset can match or outperform agents trained on much larger datasets. Surprisingly, we observe that agents trained on just 122 scenes from our dataset outperform agents trained on 10,000 scenes from the ProcTHOR-10K dataset in terms of zero-shot generalization in real-world scanned environments.

==> tables/fp_vs_pt_122.tex <==
\begin{table}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{} lcc cc @{}}
\toprule
Eval dataset $\rightarrow$ & \multicolumn{2}{c}{MP3D} & \multicolumn{2}{c}{HM3DSem} \\
\cmidrule(l{0pt}r{2pt}){2-3} \cmidrule(l{2pt}r{2pt}){4-5} 
Train dataset $\downarrow$ & Success $\uparrow$ & SPL $\uparrow$ & Success $\uparrow$ & SPL $\uparrow$ \\

\midrule

ProcTHOR-5K & 7.19 \stderr{1.1} * & 2.59 \stderr{0.16} * & 11.47 \stderr{1.08} & 4.39 \stderr{0.35} \\
ProcTHOR-10K & 8.26 \stderr{0.73} * & 2.96 \stderr{0.46} * & 12.53 \stderr{0.49} & 5.26 \stderr{0.2} \\
\midrule

ProcTHOR-60 & 3.34 \stderr{0.7} & 1.17 \stderr{0.21} & 8.08 \stderr{0.67} & 3.09 \stderr{0.28}  \\
\ourdataset-60 & 12.41 \stderr{0.79} & 4.88 \stderr{0.16} & 17.44 \stderr{1.86} & 6.73 \stderr{0.64} \\
\midrule

ProcTHOR-122 & 5.47 \stderr{1.27} & 1.83 \stderr{0.39} & 9.33 \stderr{2.19} & 3.47 \stderr{0.66}  \\

\ourdataset-122 & 14.44 \stderr{1.29} * & 5.17 \stderr{0.48} * & 19.15 \stderr{0.95} & 7.71 \stderr{0.47} \\
\bottomrule
\end{tabular}}
\caption{
\textbf{Performance of agents trained on scale-matched ProcTHOR and \ourdataset and evaluated on HM3DSem and MP3D.}
We compare agents trained on \ourdataset and a scale-matched set of 122 ProcTHOR scenes with and without finetuning.
With equal scene dataset sizes, \ourdataset leads to better agent performance in both zero-shot and fine-tuned settings.
The higher visual fidelity and correlation to HM3DSem of \ourdataset scenes are likely contributing to this improved performance. \todo{We can remove this table like last time – and just showcase numbers through figure 6.}
}
\label{tab:fp_vs_pt-122}
\end{table}


==> tables/fp_vs_pt_122_old.tex <==
\begin{table}
\centering
\begin{tabular}{@{} llcc @{}}
\toprule
Evaluation & Train dataset & Success $\uparrow$ & SPL $\uparrow$ \\
\midrule
\multirow{2}{*}{Zero-shot}
& ProcTHOR-122 & 13 \stderr{1.03} & 6 \stderr{0.51}  \\
& \ourdataset-122 & \best{19} \stderr{1.19} & \best{7} \stderr{0.48} \\
\midrule
\multirow{2}{*}{Fine-tuned}
& ProcTHOR-122 & 46 \stderr{1.52} & 21 \stderr{0.85} \\
& \ourdataset-122 & 46 \stderr{1.52} & \best{22} \stderr{0.86}\\
\bottomrule
\end{tabular}
\caption{
\textbf{Performance of agents trained on scale-matched \ourdataset and ProcTHOR and evaluated on HM3DSem.}
We compare agents trained on \ourdataset and a scale-matched set of 122 ProcTHOR scenes with and without finetuning.
With equal scene dataset sizes, \ourdataset leads to better agent performance in both zero-shot and fine-tuned settings.
The higher visual fidelity and correlation to HM3DSem of \ourdataset scenes are likely contributing to this improved performance.
}
\label{tab:fp_vs_pt-122}
\end{table}


==> tables/transfer_finetune.tex <==
\begin{table}
\centering
\begin{tabular}{@{} lcc @{}}
\toprule
Train dataset & Success $\uparrow$ & SPL $\uparrow$ \\
\midrule
ProcTHOR-10K & 45 \stderr{1.52} & 21 \stderr{0.87}  \\
\ourdataset-122 & \best{46} \stderr{1.52} & \best{22} \stderr{0.86} \\
\bottomrule
\end{tabular}
\caption{
\textbf{ObjectNav performance after fine-tuning on HM3DSem.}
We fine-tune agents trained on \ourdataset and ProcTHOR-10K on the HM3DSem train set.
The reported performance is on the HM3DSem val set.
We see that the much smaller \ourdataset-122 leads to agents that are better initialized for fine-tuning than ProcTHOR-10K.
}
\label{tab:fine_6_28}
\end{table}


==> tables/transfer_zero_old.tex <==
\begin{table*}
\centering
{%
\begin{tabular}{@{} lccccccc cc @{}}
\toprule
Eval dataset $\rightarrow$ & \multicolumn{2}{c}{iTHOR} & \multicolumn{2}{c}{ProcTHOR} &
  \multicolumn{2}{c}{\ourdataset} & \multicolumn{2}{c}{HM3DSem} \\
\cmidrule(l{0pt}r{2pt}){2-3} \cmidrule(l{2pt}r{2pt}){4-5} \cmidrule(l{2pt}r{2pt}){6-7} \cmidrule(l{2pt}r{0pt}){8-9}
Train dataset $\downarrow$ & Success $\uparrow$ & SPL $\uparrow$ & Success $\uparrow$ & SPL $\uparrow$ & Success $\uparrow$ & SPL $\uparrow$ & Success $\uparrow$ & SPL $\uparrow$ \\
\midrule
iTHOR & 70 \stderr{2.49} & \best{46} \stderr{1.88} & 32 \stderr{0.52} & 18 \stderr{0.33} & 17 \stderr{1.09} & 8 \stderr{0.58} & 12 \stderr{0.98} & 5 \stderr{0.44}\\
ProcTHOR-10K & 69 \stderr{2.51} & 42 \stderr{1.82} & \best{78} \stderr{0.46} & \best{47} \stderr{0.35} & 33 \stderr{1.36} & 14 \stderr{0.67} & 17 \stderr{1.15} & \best{7} \stderr{0.53} \\
\ourdataset-122 & \best{73} \stderr{2.43} & 33 \stderr{1.57} & 42 \stderr{0.55} & 17 \stderr{0.27} & \best{48} \stderr{1.45} & \best{21} \stderr{0.75} & \best{19} \stderr{1.19} & \best{7} \stderr{0.48} \\
\midrule
HM3DSem & 21 \stderr{2.23} & 6 \stderr{0.73} & 13 \stderr{0.36} & 5 \stderr{0.17} & 14 \stderr{1.01} & 5 \stderr{0.4} & 46 \stderr{1.52} & 20 \stderr{0.8} \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{ObjectNav zero-shot generalization across datasets.}
Agents are trained on the training set of the dataset indicated in each row and evaluated on the val set of the datasets in the columns.
As expected, agents perform well when evaluated on the dataset on which they were trained.
When looking at the generalization trends, we observe that surprisingly \ourdataset-122 achieves comparable or better generalization performance on HM3DSem compared to the much larger scale ProcTHOR-10K.
}
\label{tab:zero_6_28}
\end{table*}

